Open Range Pitch Tracking for Carrier Frequency Difference Estimation from HF Transmitted Speech

In this paper we investigate the task of detecting carrier frequency differences from demodulated single sideband signals by examining the pitch contours of the received baseband speech signal in the short-time spectral domain. From the detected pitch frequency trajectory and its harmonics a carrier frequency difference, which is caused by demodulating the radio signal with the wrong carrier frequency, can be deduced. A computationally efficient realization in the power cepstral domain is presented. The core component, i.e., the pitch tracking algorithm, is shown to perform comparably to a state of the art algorithm. The full carrier frequency difference estimation system is tested on recordings of real transmissions over HF links. A comparison with an existing approach shows improved estimation accuracy, both on short and longer speech utterances

==> sections/dnn.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = ./../SchPitch.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Deep Neural Network}\label{SEC:DNN}
The proposed approach can be further improved by exchanging the two maximum operations of \eqref{EQ:Max} and \eqref{EQ:Argmax} by a \gls{DNN} based detector directly working on the features $\bm{\Gamma}(t,\bm{f}_{P},f_{S})$.

From the \gls{DNN} we expect that it learns the temporal dependencies ...



